Multiple View Neural Regression of a Facial Shape Model

Creating re-topologized 3D facial meshes is essential for high-quality facial animation but remains labor-intensive and time-consuming. This dissertation explores more efficient approaches for capturing production-ready facial meshes through: (1) the development of VarIS, a custom light sphere for capturing high-resolution stereo geometry and reflectance maps; (2) analysis of camera parameters affecting automatic 2D and 3D landmarking; (3) synthetic-data methods for training neural face regression; and (4) techniques for improving neural multi-view face-shape regression. While VarIS enables photorealistic face capture, its operational and processing costs motivate a more scalable approach. A deep learning framework is therefore proposed to directly predict re-topologized facial meshes from synthetic multiview images generated with Visage Craft, an in-house physically based rendering system using an Appearance 3D Morphable Model (A3DMM). The system produces standardized meshes ready for rigging and animation with minimal human supervision. Results show that incorporating accurate camera intrinsics and extrinsics improves landmark accuracy and geometric consistency, while 3D landmark regularization further improves reconstruction quality.

==> 3dmm.tex <==
\chapter{Appearance 3D Morphable Model}
Deep neural networks have recently made it possible to learn retopologized meshes directly from images without the need for intermediate processes. We contend that facial image acquisition is a core task in developing deep learning-based digital avatars. Previous approaches for learning facial models from images have either relied on large datasets of real people captured in controlled environments or constructed datasets from single human face images using statistical models. In contrast, An Appearance 3D Morphable Model (A3DMM) is built from a small set of scans of individuals' faces and used with physically based shading and random generation to create a synthetic dataset, using our software Visage Craft.

\section{Visage Craft: Countenance Lab Active 3D Morphable Model }



\section{Cinematic Rendering Faces in Unreal Engine 5.3}
In April 2022, Epic Games introduced Unreal Engine 5.0, unveiling Metahuman—a remarkable creation featuring intricately detailed and realistic digital characters. Leveraging cutting-edge facial scanning, rigging, and animation technologies, Metahumans achieve unprecedented lifelike visual fidelity.  Users have the flexibility to import facial meshes and transform them into personalized Metahuman characters, allowing for stylization choices such as hairstyle and skin color. Furthermore, Unreal Engine provides an advanced rendering system, enabling the generation of photorealistic images of human faces. We acquired 70 faces from the 3D Scan Store, including various genders, ages, and ethnicities. Subsequently, we manually converted all the scans to Metahuman characters and applied stylizations to enhance features like eyes, hair, and eyebrows. This method enables the creation of higher-fidelity, more realistic faces complete with eyes and hair, and facilitates the generation of multiple facial expressions compared to other synthetic training data. Leveraging the fact that Metahuman faces are pre-rigged, performance captures can be efficiently conducted for all facial scans. Figure \ref{fig:metahuman} shows a sample of faces rendered in the Unreal Engine.




\begin{figure}[h!]
    \centering
    \includegraphics[width=0.8\linewidth]{figure/metahuman.png}
    \caption{Unreal Engine Rendered Metahuman Faces}
    \label{fig:metahuman}
\end{figure}


==> remainWork.tex <==
\chapter{Remaining Work}

Having implemented various neural network architectures, the next step entails testing the deep learning retopology system using images acquired from our custom Variable Illumination Sphere (VarIS). These tests are conducted under the same camera settings as those utilized in generating the synthetic training dataset. To expedite the testing phase, we could augment the dataset by generating photorealistic data from Unreal Engine using Metahuman. Additionally, the integration of an Active 3D Morphable Model in Unreal Engine may enable the generation of more photorealistic human face images as a neural network training corpus.


\subsection{Revising Neural Network Architectures}

As previously outlined, the two neural network architectures will be reexamined. In the conventional autoencoder training process, the latent vector is typically resampled using a probability distribution, commonly the normal distribution, a technique known as the parameterization trick. To enhance the training process, statistics eigenvalues derived from the principal component decomposition of the scanned faces will be incorporated into the variational autoencoder architectures. This inclusion aims to expedite the training process by providing constraints on each dimension of the latent vector.

Over the recent years, the transformer deep learning architecture has garnered significant research attention. We will explore the transformer neural network, as it exhibits faster convergence and produces results as good as the other approaches.


\subsection{Automate Unreal Engine Metahuman Groundtruth Generation}
An automatic generation of multi-viewpoint renders in the Unreal Engine using high-fidelity Metahuman face scans is currently under development. The 3D scan meshes could also be used as ground truth to validate neural network results.

==> summary.tex <==
%
% summary.tex
% Collect this during your research to organize thoughts and references and to force yourself to organize and create your .bib file ahead of time.  Then you can copy and paste these in order to fill out your outline for your background and related work sections.
%

%  Use a chapter just for this simple summary file to display title at top.    
\chapter*{Summary for Thesis Project:  }    
    
% can use these sections as desired to help organize content    
\section{Reference Item Titled to Help Remember Its Content}

This is an example of a summary with a citation~\cite{aror:alits}.  Include a few sentences to a paragraph or however many needed to summarize effectively papers and other references.  Go ahead and add the entries to your bib file so that you may cite them here.  These paragraphs may be copied, re-arranged, and edited to begin your background work section of your thesis.  Add at least one for each reference.  New paragraphs may be made simply by leaving some white space between.  If there are meaningful figures from papers, you may wish to go ahead and collect those separately in an images folder or make note of them in your summary paragraphs.


\section{This Could Be a Second Reference}

This is an example of a summary with a citation~\cite{aror:alits}.  Include a few sentences to a paragraph or however many needed to summarize effectively papers and other references.  Go ahead and add the entries to your bib file so that you may cite them here.  These paragraphs may be copied, re-arranged, and edited to begin your background work section of your thesis.  Add at least one for each reference.  New paragraphs may be made simply by leaving some white space between.

                              

%  Make sure to include bib entries in the .bib file for all of your references as you find, research, and write this summary document.

